3DGTN: 3D Dual-Attention GLocal Transformer Network for Point Cloud Classification and Segmentation

Although the application of Transformers in 3D point cloud processing has achieved significant progress and success, it is still challenging for existing 3D Transformer methods to efficiently and accurately learn both valuable global features and valuable local features for improved applications. This paper presents a novel point cloud representational learning network, called 3D Dual Self-attention Global Local (GLocal) Transformer Network (3DGTN), for improved feature learning in both classification and segmentation tasks, with the following key contributions. First, a GLocal Feature Learning (GFL) block with the dual self-attention mechanism (i.e., a novel Point-Patch Self-Attention, called PPSA, and a channel-wise self-attention) is designed to efficiently learn the GLocal context information. Second, the GFL block is integrated with a multi-scale Graph Convolution-based Local Feature Aggregation (LFA) block, leading to a Global-Local (GLocal) information extraction module that can efficiently capture critical information. Third, a series of GLocal modules are used to construct a new hierarchical encoder-decoder structure to enable the learning of "GLocal" information in different scales in a hierarchical manner. The proposed framework is evaluated on both classification and segmentation datasets, demonstrating that the proposed method is capable of outperforming many state-of-the-art methods on both classification and segmentation tasks.

==> bib_copy.tex <==
%#####################################voxel######################################################
@inproceedings{wu20153d,
  title={3d shapenets: A deep representation for volumetric shapes},
  author={Wu, Zhirong and Song, Shuran and Khosla, Aditya and Yu, Fisher and Zhang, Linguang and Tang, Xiaoou and Xiao, Jianxiong},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1912--1920},
  year={2015}
}

@inproceedings{maturana2015voxnet,
  title={Voxnet: A 3d convolutional neural network for real-time object recognition},
  author={Maturana, Daniel and Scherer, Sebastian},
  booktitle={2015 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={922--928},
  year={2015},
  organization={IEEE}
}

@inproceedings{riegler2017octnet,
  title={Octnet: Learning deep 3d representations at high resolutions},
  author={Riegler, Gernot and Osman Ulusoy, Ali and Geiger, Andreas},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3577--3586},
  year={2017}
}

@article{atzmon2018point,
  title={Point convolutional neural networks by extension operators},
  author={Atzmon, Matan and Maron, Haggai and Lipman, Yaron},
  journal={arXiv preprint arXiv:1803.10091},
  year={2018}
}

@inproceedings{le2018pointgrid,
  title={Pointgrid: A deep network for 3d shape understanding},
  author={Le, Truc and Duan, Ye},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={9204--9214},
  year={2018}
}

@inproceedings{choy20194d,
  title={4d spatio-temporal convnets: Minkowski convolutional neural networks},
  author={Choy, Christopher and Gwak, JunYoung and Savarese, Silvio},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3075--3084},
  year={2019}
}

%#####################################projection######################################################

@inproceedings{su2015multi,
  title={Multi-view convolutional neural networks for 3d shape recognition},
  author={Su, Hang and Maji, Subhransu and Kalogerakis, Evangelos and Learned-Miller, Erik},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={945--953},
  year={2015}
}

@inproceedings{chen2017multi,
  title={Multi-view 3d object detection network for autonomous driving},
  author={Chen, Xiaozhi and Ma, Huimin and Wan, Ji and Li, Bo and Xia, Tian},
  booktitle={Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
  pages={1907--1915},
  year={2017}
}

@inproceedings{kanezaki2018rotationnet,
  title={Rotationnet: Joint object categorization and pose estimation using multiviews from unsupervised viewpoints},
  author={Kanezaki, Asako and Matsushita, Yasuyuki and Nishida, Yoshifumi},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5010--5019},
  year={2018}
}

@inproceedings{tatarchenko2018tangent,
  title={Tangent convolutions for dense prediction in 3d},
  author={Tatarchenko, Maxim and Park, Jaesik and Koltun, Vladlen and Zhou, Qian-Yi},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3887--3896},
  year={2018}
}

@article{zhang20183d,
  title={3D Point Cloud Recognition Based on a Multi-View Convolutional Neural Network},
  author={Zhang, Le and Sun, Jian and Zheng, Qiang},
  journal={Sensors},
  volume={18},
  number={11},
  pages={3681},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{wei2020view,
  title={View-GCN: View-based graph convolutional network for 3D shape analysis},
  author={Wei, Xin and Yu, Ruixuan and Sun, Jian},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1850--1859},
  year={2020}
}

@article{yu20213d,
  title={3D object representation learning: A set-to-set matching perspective},
  author={Yu, Tan and Meng, Jingjing and Yang, Ming and Yuan, Junsong},
  journal={IEEE Transactions on Image Processing},
  volume={30},
  pages={2168--2179},
  year={2021},
  publisher={IEEE}
}

%#####################################point-based######################################################

@inproceedings{qi2017pointnet,
  title={Pointnet: Deep learning on point sets for 3d classification and segmentation},
  author={Qi, Charles R and Su, Hao and Mo, Kaichun and Guibas, Leonidas J},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={652--660},
  year={2017}
}

@article{qi2017pointnet++,
  title={Pointnet++: Deep hierarchical feature learning on point sets in a metric space},
  author={Qi, Charles R and Yi, Li and Su, Hao and Guibas, Leonidas J},
  journal={arXiv preprint arXiv:1706.02413},
  year={2017}
}

@inproceedings{paigwar2019attentional,
  title={Attentional pointnet for 3d-object detection in point clouds},
  author={Paigwar, Anshul and Erkent, Ozgur and Wolf, Christian and Laugier, Christian},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={0--0},
  year={2019}
}

@inproceedings{qi2018frustum,
  title={Frustum pointnets for 3d object detection from rgb-d data},
  author={Qi, Charles R and Liu, Wei and Wu, Chenxia and Su, Hao and Guibas, Leonidas J},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={918--927},
  year={2018}
}

@article{li2018pointcnn,
  title={Pointcnn: Convolution on x-transformed points},
  author={Li, Yangyan and Bu, Rui and Sun, Mingchao and Wu, Wei and Di, Xinhan and Chen, Baoquan},
  journal={Advances in neural information processing systems},
  volume={31},
  pages={820--830},
  year={2018}
}

@inproceedings{wu2019pointconv,
  title={Pointconv: Deep convolutional networks on 3d point clouds},
  author={Wu, Wenxuan and Qi, Zhongang and Fuxin, Li},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9621--9630},
  year={2019}
}

@article{wang2019dynamic,
  title={Dynamic graph cnn for learning on point clouds},
  author={Wang, Yue and Sun, Yongbin and Liu, Ziwei and Sarma, Sanjay E and Bronstein, Michael M and Solomon, Justin M},
  journal={Acm Transactions On Graphics (tog)},
  volume={38},
  number={5},
  pages={1--12},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{simonovsky2017dynamic,
  title={Dynamic edge-conditioned filters in convolutional neural networks on graphs},
  author={Simonovsky, Martin and Komodakis, Nikos},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3693--3702},
  year={2017}
}

@inproceedings{lin2020convolution,
  title={Convolution in the cloud: Learning deformable kernels in 3d graph convolution networks for point cloud analysis},
  author={Lin, Zhi-Hao and Huang, Sheng-Yu and Wang, Yu-Chiang Frank},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1800--1809},
  year={2020}
}

@inproceedings{li2019deepgcns,
  title={Deepgcns: Can gcns go as deep as cnns?},
  author={Li, Guohao and Muller, Matthias and Thabet, Ali and Ghanem, Bernard},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9267--9276},
  year={2019}
}

@inproceedings{liu2019point2sequence,
  title={Point2sequence: Learning the shape representation of 3d point clouds with an attention-based sequence to sequence network},
  author={Liu, Xinhai and Han, Zhizhong and Liu, Yu-Shen and Zwicker, Matthias},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={8778--8785},
  year={2019}
}
%#####################################Transformer-based######################################################
@inproceedings{hui2021pyramid,
  title={Pyramid Point Cloud Transformer for Large-Scale Place Recognition},
  author={Hui, Le and Yang, Hang and Cheng, Mingmei and Xie, Jin and Yang, Jian},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={6098--6107},
  year={2021}
}

@article{engel2021point,
  title={Point transformer},
  author={Engel, Nico and Belagiannis, Vasileios and Dietmayer, Klaus},
  journal={IEEE Access},
  volume={9},
  pages={134826--134840},
  year={2021},
  publisher={IEEE}
}

@article{guo2021pct,
  title={Pct: Point cloud transformer},
  author={Guo, Meng-Hao and Cai, Jun-Xiong and Liu, Zheng-Ning and Mu, Tai-Jiang and Martin, Ralph R and Hu, Shi-Min},
  journal={Computational Visual Media},
  volume={7},
  number={2},
  pages={187--199},
  year={2021},
  publisher={Springer}
}

@inproceedings{zhao2021point,
  title={Point transformer},
  author={Zhao, Hengshuang and Jiang, Li and Jia, Jiaya and Torr, Philip HS and Koltun, Vladlen},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={16259--16268},
  year={2021}
}

@article{han2021point,
  title={Point Cloud Learning with Transformer},
  author={Han, Xian-Feng and Kuang, Yu-Jia and Xiao, Guo-Qiang},
  journal={arXiv preprint arXiv:2104.13636},
  year={2021}
}

@article{qiu2021pu,
  title={PU-Transformer: Point Cloud Upsampling Transformer},
  author={Qiu, Shi and Anwar, Saeed and Barnes, Nick},
  journal={arXiv preprint arXiv:2111.12242},
  year={2021}
}

@article{bruna2013spectral,
  title={Spectral networks and locally connected networks on graphs},
  author={Bruna, Joan and Zaremba, Wojciech and Szlam, Arthur and LeCun, Yann},
  journal={arXiv preprint arXiv:1312.6203},
  year={2013}
}

@article{engel2020point,
  title={Point transformer},
  author={Engel, Nico and Belagiannis, Vasileios and Dietmayer, Klaus},
  journal={arXiv preprint arXiv:2011.00931},
  year={2020}
}

@inproceedings{yang2019modeling,
  title={Modeling point clouds with self-attention and gumbel subset sampling},
  author={Yang, Jiancheng and Zhang, Qiang and Ni, Bingbing and Li, Linguo and Liu, Jinxian and Zhou, Mengdie and Tian, Qi},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3323--3332},
  year={2019}
}

@article{gao2022lft,
  title={LFT-Net: Local Feature Transformer Network for Point Clouds Analysis},
  author={Gao, Yongbin and Liu, Xuebing and Li, Jun and Fang, Zhijun and Jiang, Xiaoyan and Huq, Kazi Mohammed Saidul},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  year={2022},
  publisher={IEEE}
}

@article{chen2019gapnet,
  title={Gapnet: Graph attention based point neural network for exploiting local feature of point cloud},
  author={Chen, Can and Fragonara, Luca Zanotti and Tsourdos, Antonios},
  journal={arXiv preprint arXiv:1905.08705},
  year={2019}
}
%#####################################VisionTransformer######################################################

@inproceedings{misra2021end,
  title={An End-to-End Transformer Model for 3D Object Detection},
  author={Misra, Ishan and Girdhar, Rohit and Joulin, Armand},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={2906--2917},
  year={2021}
}

@inproceedings{mazur2021cloud,
  title={Cloud transformers: A universal approach to point cloud processing tasks},
  author={Mazur, Kirill and Lempitsky, Victor},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={10715--10724},
  year={2021}
}

@inproceedings{zhou2016learning,
  title={Learning deep features for discriminative localization},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2921--2929},
  year={2016}
}

@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

@article{wu2021cvt,
  title={Cvt: Introducing convolutions to vision transformers},
  author={Wu, Haiping and Xiao, Bin and Codella, Noel and Liu, Mengchen and Dai, Xiyang and Yuan, Lu and Zhang, Lei},
  journal={arXiv preprint arXiv:2103.15808},
  year={2021}
}

@article{liu2021swin,
  title={Swin transformer: Hierarchical vision transformer using shifted windows},
  author={Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  journal={arXiv preprint arXiv:2103.14030},
  year={2021}
}

@inproceedings{zhao2020exploring,
  title={Exploring self-attention for image recognition},
  author={Zhao, Hengshuang and Jia, Jiaya and Koltun, Vladlen},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10076--10085},
  year={2020}
}

@inproceedings{ranftl2021vision,
  title={Vision transformers for dense prediction},
  author={Ranftl, Ren{\'e} and Bochkovskiy, Alexey and Koltun, Vladlen},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={12179--12188},
  year={2021}
}

@article{yuan2021tokens,
  title={Tokens-to-token vit: Training vision transformers from scratch on imagenet},
  author={Yuan, Li and Chen, Yunpeng and Wang, Tao and Yu, Weihao and Shi, Yujun and Jiang, Zihang and Tay, Francis EH and Feng, Jiashi and Yan, Shuicheng},
  journal={arXiv preprint arXiv:2101.11986},
  year={2021}
}

@article{wang2021pyramid,
  title={Pyramid vision transformer: A versatile backbone for dense prediction without convolutions},
  author={Wang, Wenhai and Xie, Enze and Li, Xiang and Fan, Deng-Ping and Song, Kaitao and Liang, Ding and Lu, Tong and Luo, Ping and Shao, Ling},
  journal={arXiv preprint arXiv:2102.12122},
  year={2021}
}

@inproceedings{wang2021end,
  title={End-to-end video instance segmentation with transformers},
  author={Wang, Yuqing and Xu, Zhaoliang and Wang, Xinlong and Shen, Chunhua and Cheng, Baoshan and Shen, Hao and Xia, Huaxia},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8741--8750},
  year={2021}
}

%#####################################investigation######################################################
@inproceedings{xie2018attentional,
  title={Attentional shapecontextnet for point cloud recognition},
  author={Xie, Saining and Liu, Sainan and Chen, Zeyu and Tu, Zhuowen},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4606--4615},
  year={2018}
}

@article{feng2020point,
  title={Point attention network for semantic segmentation of 3D point clouds},
  author={Feng, Mingtao and Zhang, Liang and Lin, Xuefei and Gilani, Syed Zulqarnain and Mian, Ajmal},
  journal={Pattern Recognition},
  volume={107},
  pages={107446},
  year={2020},
  publisher={Elsevier}
}

@article{qiu2021geometric,
  title={Geometric back-projection network for point cloud classification},
  author={Qiu, Shi and Anwar, Saeed and Barnes, Nick},
  journal={IEEE Transactions on Multimedia},
  year={2021},
  publisher={IEEE}
}
%#####################################comaprison######################################################

@inproceedings{qi2016volumetric,
  title={Volumetric and multi-view cnns for object classification on 3d data},
  author={Qi, Charles R and Su, Hao and Nie{\ss}ner, Matthias and Dai, Angela and Yan, Mengyuan and Guibas, Leonidas J},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={5648--5656},
  year={2016}
}

@article{lin2021diffconv,
  title={diffConv: Analyzing Irregular Point Clouds with an Irregular View},
  author={Lin, Manxi and Feragen, Aasa},
  journal={arXiv preprint arXiv:2111.14658},
  year={2021}
}

@inproceedings{zhao2019pointweb,
  title={Pointweb: Enhancing local neighborhood features for point cloud processing},
  author={Zhao, Hengshuang and Jiang, Li and Fu, Chi-Wing and Jia, Jiaya},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5565--5573},
  year={2019}
}

@article{muzahid2020curvenet,
  title={Curvenet: Curvature-based multitask learning deep networks for 3D object recognition},
  author={Muzahid, AAM and Wan, Wanggen and Sohel, Ferdous and Wu, Lianyao and Hou, Li},
  journal={IEEE/CAA Journal of Automatica Sinica},
  volume={8},
  number={6},
  pages={1177--1187},
  year={2020},
  publisher={IEEE}
}

@inproceedings{kaul2021fatnet,
  title={FatNet: A feature-attentive network for 3D point cloud processing},
  author={Kaul, Chaitanya and Pears, Nick and Manandhar, Suresh},
  booktitle={2020 25th International Conference on Pattern Recognition (ICPR)},
  pages={7211--7218},
  year={2021},
  organization={IEEE}
}

@inproceedings{uy2019revisiting,
  title={Revisiting point cloud classification: A new benchmark dataset and classification model on real-world data},
  author={Uy, Mikaela Angelina and Pham, Quang-Hieu and Hua, Binh-Son and Nguyen, Thanh and Yeung, Sai-Kit},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={1588--1597},
  year={2019}
}

@inproceedings{qiu2021dense,
  title={Dense-resolution network for point cloud classification and segmentation},
  author={Qiu, Shi and Anwar, Saeed and Barnes, Nick},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={3813--3822},
  year={2021}
}

@article{lai2022stratified,
  title={Stratified Transformer for 3D Point Cloud Segmentation},
  author={Lai, Xin and Liu, Jianhui and Jiang, Li and Wang, Liwei and Zhao, Hengshuang and Liu, Shu and Qi, Xiaojuan and Jia, Jiaya},
  journal={arXiv preprint arXiv:2203.14508},
  year={2022}
}

@article{fu2022distillation,
  title={Distillation with Contrast is All You Need for Self-Supervised Point Cloud Representation Learning},
  author={Fu, Kexue and Gao, Peng and Zhang, Renrui and Li, Hongsheng and Qiao, Yu and Wang, Manning},
  journal={arXiv preprint arXiv:2202.04241},
  year={2022}
}

@article{palazzi2018predicting,
  title={Predicting the Driver's Focus of Attention: the DR (eye) VE Project},
  author={Palazzi, Andrea and Abati, Davide and Solera, Francesco and Cucchiara, Rita and others},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={41},
  number={7},
  pages={1720--1733},
  year={2018},
  publisher={IEEE}
}
